SpDISTAL: Compiling Distributed Sparse Tensor Computations

We introduce SpDISTAL, a compiler for sparse tensor algebra that targets distributed systems. SpDISTAL combines separate descriptions of tensor algebra expressions, sparse data structures, data distribution, and computation distribution. Thus, it enables distributed execution of sparse tensor algebra expressions with a wide variety of sparse data structures and data distributions. SpDISTAL is implemented as a C++ library that targets a distributed task-based runtime system and can generate code for nodes with both multi-core CPUs and multiple GPUs. SpDISTAL generates distributed code that achieves performance competitive with hand-written distributed functions for specific sparse tensor algebra expressions and that outperforms general interpretation-based systems by one to two orders of magnitude.

==> old-codegen-section.tex <==
\section{Composing Sparse Data Structures With Distribution Primitives}\label{sec:algorithms}

A key contribution of \name{} is a compiler technique that realizes the
%sparse distributed 
programming model discussed in \autoref{sec:programming-model}.
%
We first discuss preliminary concepts and terminology before describing our
compilation approach.

\subsection{Preliminaries}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/coord-tree}
    \caption{Coordinate tree representation of a sparse matrix.}
    \label{fig:coord-tree}
\end{figure}

\emph{Coordinate Trees.}
%
The \emph{coordinate tree} representation of a tensor $\mT$ is a tree with one level per
dimension of $\mT$ (in addition to a root), as show in \autoref{fig:coord-tree}.
%
Each tree path from the root to a leaf node represents a non-zero tensor coordinate.
%
The levels of the coordinate tree are ordered in the way the dimensions of $\mT$ are stored.
%
For example, a row-major layout of a matrix would have rows followed by columns, while
a column-major layout would have columns followed by rows.

\emph{Format Abstraction.}
%
In \name{}, each tensor dimension is encoded by a user-specified \emph{level format} that
encodes how the data in a coordinate tree level is physically stored in memory.
%
Chou et al.~\cite{taco_formats} proposed a compile-time interface for level formats that provides
an abstraction for a code generation algorithm to target.
%
The abstraction allows new formats implementing the interface to be added without
changing the code generation algorithm.
%
The format abstraction consists of functions that return intermediate representation (IR) fragments
that the code generator can utilize to generate code specialized to tensor level formats.
%(i.e. how to access an encoded coordinate while iterating over a \compressed{} level.)
%
We refer to the functions that a level implements as part of the format abstraction
as \emph{level functions}.

\emph{Iteration Kinds.}
%
TACO breaks iteration over sparse loops into two kinds: \emph{coordinate value} iteration and \emph{coordinate position} iteration.
%
Coordinate value loops iterate over all values of 
a coordinate, corresponding to a dense \texttt{for} loop.
%
Coordinate position loops instead iterate over only the non-zero
coordinates in a level by directly iterating over the positions in 
the sparse data structure that hold non-zero coordinates in the level.

\subsection{Partitioning}

Describing how data structures are \emph{partitioned} is a key problem
in distributing a computation.
%
However, the irregular data structures that encode sparse tensors 
makes this process difficult.
%
Through a novel compilation techniques, we describe a procedure
to derive partitions of sparse tensors for a target computation
or data placement operation.

% \begin{figure}[t]
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/coord-tree-univ-part-top-level}
%         \caption{Universe partition of level one.}
%         \label{fig:coord-tree-univ-part-top-level}
%     \end{subfigure}\hfill
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/coord-tree-coord-part-top-level}
%         \caption{Non-zero partition of level two.}
%         \label{fig:coord-tree-coord-part-top-level}
%     \end{subfigure}\hfill
%     \caption{Initial level partitions of coordinate trees.}
%     \label{fig:coord-tree-top-level-parts}
% \end{figure}

\begin{figure}[t]
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/coord-tree-full-univ-part}
        \caption{Universe partition of level one.}
        \label{fig:coord-tree-univ-full-part}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/coord-tree-full-coord-part}
        \caption{Non-zero partition of level two.}
        \label{fig:coord-tree-full-coord-part}
    \end{subfigure}
    \caption{Coordinate tree partitions derived from a level partition. Dashed grey lines indicate
    the initial level partition.}
    \label{fig:coord-tree-full-parts}
\end{figure}

\emph{Intuition.}
%
To build intuition for the partitioning process, we appeal to the coordinate
tree representation of a sparse tensor.
%
Consider the row-based and non-zero-based SpMV algorithms
discussed in \autoref{sec:programming-model:spmv}.
%
The distributed loop iterations correspond to a 
partition of the matrix's coordinate tree.
%
The first strategy distributed the rows, and corresponds to a partition
of the first coordinate tree level (\autoref{fig:coord-tree-univ-full-part}).
%
The second strategy distributes the non-zero coordinates, corresponding
to a partition of the second coordinate tree level (\autoref{fig:coord-tree-full-coord-part}).
%
In the row-based strategy, each coordinate in the first dimension of
the matrix will access all child coordinates in the second dimension of the tree.
%
In the non-zero based strategy, each coordinate in the second dimension of
the matrix needs to access its parent coordinate in the first dimension of the tree.

\autoref{fig:coord-tree-univ-full-part} and \autoref{fig:coord-tree-full-coord-part} depict
the full coordinate tree partitions for each of the distribution strategies.
%
Given a partitioning of coordinate tree level, we can obtain a partition
of the child level by applying the partition to the children of each node in the level.
%
Conversely, we can obtain a partition of the parent level of a partitioned
level by partitioning the parent level such that each parent node is colored with all of the colors
of its children.
%
%This intuition is similar to the dependent partitioning framework proposed by Treichler et al.~\cite{deppart},
%where applications tend to compute an "initial" partition, and then derive "dependent" partitions
%of the remaining program data.

\emph{Data Structures.}
%
In order to develop the coordinate tree intuition in a concrete approach, we first describe abstract
data structures that our generated code will manipulate, and then use these structures
to encode the level formats.
%
A \emph{region} is a distributed multi-dimensional array of values.
%
An \emph{index space} is an abstract object that represents the set of indices of a region.
%
A \emph{partition} is an object that represents a mapping from a set of \emph{colors}
to (potentially overlapping) subsets of an index space.
%
A region can be \emph{partitioned} into \emph{sub-regions} by partitioning the index space
corresponding to the region's indices.

Key operations on partitions are \emph{image} and \emph{preimage}, 
which can be applied to partitions of regions that contain index sets as values.
%
These operations are \emph{dependent partitioning} operations, as they create
new partitions from existing partitions.

Consider an index space $I$ and a region $R$ where each element of $R$ is a subset of $I$.
%
Given a partition $P$ of $R$, \texttt{image(P, R)} is a partition $P'$ of $I$
such that $\forall c \in P, \forall i \in P[c], R[i] \subseteq P'[c]$, depicted in
\autoref{fig:deppart-image}.

The preimage operation is the inverse of image.
%
Consider an index space $I$ and a target region $R$ where each element of $R$ is a subset of $I$.
%
Given a partition $P$ of $I$, the \texttt{preimage(P, R)} is a partition
$P'$ of $R$ such that $\forall c \in P, \forall i \in P[c], \forall i'~\textsf{s.t.}~i \in R[i'], i' \in P'[c]$, depicted in \autoref{fig:deppart-preimage}.
%
Intuitively, the preimage operation colors
all of the in-pointers to an index space point with the same color as the point.

\begin{figure}
    \begin{subfigure}[b]{0.5\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{figures/deppart-image}
        \caption{Image}
        \label{fig:deppart-image}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.5\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{figures/deppart-preimage}
        \caption{Preimage}
        \label{fig:deppart-preimage}
    \end{subfigure}\hfill
    \caption{Visualization of image and preimage operations.}
    \label{fig:deppart-example}
\end{figure}

In order to enable partitioning and distributed computation over sparse tensors,
we now encode sparse tensors using these abstract data structures.
%
These encodings are similar to those proposed by TACO but deviate slightly
to play nicely with partitioning operations.
%
First, we explicitly encode \dense{} levels with a index space
over a domain equal to the size of the dense level, named \lstinline[basicstyle=\ttfamily\footnotesize]{dom}.
%
Next, multiple contiguous \dense{} levels are collapsed into a single
logical multi-dimensional \dense{} level that is represented by a
multi-dimensional index space.
%
In TACO, \compressed{} levels are encoded with an array of coordinates
(\crd{}) and an array that stores bounds on the range of coordinates
associated with each entry in the parent level (\pos{}).
%
In particular, the coordinates for an entry $i$ are stored in positions 
\lstinline[basicstyle=\ttfamily\footnotesize]{[pos[i], pos[i+1])}
of \crd{}.
%
We store the \pos{} and \crd{} arrays as regions in order to enable
partitioning and distribution.
%
As the \pos{} region contains pointers to ranges of the \crd{} region, our
goal is to utilize image and preimage.
%
Therefore, we store tuples in the \pos{} region that contain the lower
and upper bounds of coordinate positions, representing a set of indices 
in the \crd{} region.
%
The coordinates for an entry $i$ are now stored in positions
\lstinline[basicstyle=\ttfamily\footnotesize]{[pos[i].lo, pos[i].hi)}
of \crd{}.
%
\autoref{fig:spdistal-csr} visualizes a CSR data structure in \name{}.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/distal-csr}
    \caption{CSR data structure in \name{}.}
    \label{fig:spdistal-csr}
\end{figure}

\emph{Format Abstractions for Partitioning.}
We introduce format abstractions to describe the processes of initial 
and dependent partition creation, allowing for definition of a code generation 
algorithm that is decoupled from level format implementations.
%
The partitioning abstraction we propose has two groups, one for creation of the initial partition
and the other for creation of the derived partitions.
%
Our code generation algorithm invokes the appropriate level functions when generating code,
allowing the algorithm to not be tied to any physical data structures.
%
All discussed level functions emit code, and optionally return symbolic values 
for use in the code generator.

There are two groups of functions for the creation of initial partitions,
corresponding to universe and non-zero partitions.
%
The universe partition group consists of three functions:
%
\begin{lstlisting}
initUniversePartition()
createUniversePartitionEntry(color, bounds)
finalizeUniversePartition() -> (partition, partition)
\end{lstlisting}
%
\lstinline{initUniversePartition} initializes any necessary data structures.
%
\lstinline{createUniversePartitionEntry} takes symbolic values of a color and a
range of coordinates in the level that should be assigned to the color and maps
the range of coordinates to the color.
%
\lstinline{finalizeUniversePartition} finalizes any necessary data structures
and returns a partition to use for partitioning parent levels
and a partition to use for partitioning child levels.
%
The universe partition functions are used when a coordinate value loop
is distributed, corresponding to a partition of the universe.

The non-zero partition group consists of three functions that mirror
the universe partition group:
%
\begin{lstlisting}
initNonZeroPartition()
createNonZeroPartitionEntry(color, bounds)
finalizeNonZeroPartition() -> (partition, partition)
\end{lstlisting}
%
\lstinline{initNonZeroPartition} and \lstinline{finalizeNonZeroPartition} are the same
as their universe partition counterparts.
%
\lstinline{createNonZeroPartitionEntry} is similar to \lstinline{createUniversePartitionEntry},
but instead takes symbolic bounds on the positions within the level that encode non-zero coordinates.
%
The non-zero partition family of level functions are used when a
coordinate position loop is distributed, corresponding to a partition 
of the level's non-zero coordinates.

There are two functions for constructing derived partitions:
\begin{lstlisting}
partitionFromParent(partition) -> partition
partitionFromChild(partition) -> partition
\end{lstlisting}
%
Each function partitions a level using an existing partition,
and returns a partition to use to partitioning child or parent levels.

These functions are implemented for \dense{} and \compressed{} levels
in \autoref{tab:level-function-impls}.
%
The initial partitioning functions for \dense{} levels directly color the coordinate
space that the \dense{} level represents, and the derived partitioning functions pass
the partition through the coordinate space.
%
The universe partitioning functions for \compressed{} levels partition the
\crd{} region by bucketing the coordinates into the ranges demarcated
by \lstinline{createUniversePartitionEntry}, while the 
non-zero partitioning functions directly partition the \crd{} region
according to the position bounds demarcated by \lstinline{createNonZeroPartitionEntry}.
%
Both use a preimage to recover a partition of the \pos{} region.
%
The derived partitioning functions partition the \pos{} and \crd{} regions
from parent and child partitions, and use image and preimage to create
partitions of the other region in the level.

\begin{table*}
    \scriptsize
    \centering
    \begin{tabular}{|c|ll|}
        \hline
        Level Type &  \multicolumn{2}{c|}{Level Function Definitions} \\
        \hline
        \multirow{2}{*}{\dense{}} & \lstinputlisting{dense-univ-parts.tex} & \lstinputlisting{dense-coord-parts.tex} \\
        \cline{2-3}
        & \lstinputlisting{dense-from-parent.tex} & \lstinputlisting{dense-from-child.tex} \\
        \hline
        \multirow{2}{*}{\compressed{}} & \lstinputlisting{compressed-univ-parts.tex} & \lstinputlisting{compressed-coord-parts.tex} \\
        \cline{2-3}
        & \lstinputlisting{compressed-from-parent.tex} & \lstinputlisting{compressed-from-child.tex} \\
        \hline
    \end{tabular}
    \caption{Partitioning level function definitions for \dense{} and \compressed{} levels.}
    \label{tab:level-function-impls}
\end{table*}

% Trying out a more high-level version of the code generation algorithm.
\subsection{Code Generation}

We now describe how partitioning related format abstraction functions are used in an
algorithm to generate code that partitions sparse tensors.
%
At each distributed loop, the algorithm generates code to create initial level partitions
of sparse tensors, and then derives partitions of the remaining coordinate tree levels.
%
Finally, the algorithm emits a distributed for loop, where each iteration of the
distributed loop is passed the corresponding set of created partitions.
%
The code generation algorithm is a recursive function called on a scheduled
tensor index notation expression and recurses on index variables in the order
given by the schedule.
%
Pseudo-code for the algorithm is given in \autoref{fig:codegen-alg}.
%
\autoref{fig:example-gen-code} contains code generated by our algorithm
for a row-based SpMV computation.

Distributed coordinate value loops distribute the space of coordinates,
corresponding to universe partitions.
%
To generate partitioning code for coordinate value loops, the algorithm
first calls \lstinline{createInitialUniversePartitions}, which 
first invokes \lstinline{initUniversePartition} for each tensor accessed
by the current index variable.
%
Next, it emits a for loop over the current index variable, and symbolically
infers upper and lower bounds on the index variable to pass to calls
to \lstinline{createUniversePartitionEntry} for each accessed tensor.
%
Finally, it completes the initial level partitioning by calling
\lstinline{finalizeUniversePartition} on each accessed tensor.
%
The algorithm then calls \lstinline{partitionCoordinateTrees}, which
takes each initial level partition and partitions the full coordinate
tree by calling \lstinline{partitionFromChild} for each level above
the initial level and calling \lstinline{partitionFromParent} for each
level below the initial level.


\subsection{Code Generation}
%
We describe our code generation algorithm that utilizes the new format abstraction functions
as pseudocode in \autoref{fig:codegen-alg}.
%
Our algorithm takes as input a scheduled tensor index notation statement and recursively
calls itself on index variables in the expression, in the order given by the schedule.
%
It returns code in a low-level imperative IR that is then further lowered into C++ and CUDA.
%
If the current index variable is not distributed, then we fall back to
the standard code generation algorithm of TACO.
%
Otherwise, the algorithm proceeds in two phases corresponding to the
two groups of partitioning functions.

The algorithm emits a loop over the current distributed index variable, 
and symbolically infers the upper and lower bounds of the 
original (root) index variable that the distributed index variable corresponds to.
%
Then, the algorithm invokes level functions to 
create an initial partition with the symbolic ranges of the current index variable.
%
In the universe partition case, the algorithm partitions each tensor accessed by 
the index variable; in the non-zero partition case, the algorithm first
partitions the tensor that the non-zero coordinates are partitioned by.

In the second phase, the algorithm derives partitions of the full coordinate tree.
%
In the universe partition case, the algorithm partitions the coordinate tree
of each partitioned tensor using \lstinline[basicstyle=\ttfamily\footnotesize]!partitionFromParent! and \lstinline[basicstyle=\ttfamily\footnotesize]!partitionFromChild!.
%
In the non-zero partition case, the algorithm does the same thing for the tensor
who's non-zero coordinates have been partitioned.
%
The algorithm then projects the top-level partition to create a universe partition
of each other tensor, and then completes the partitions of those tensors.
%
\autoref{fig:codegen-partitions} visualizes the partitions created by our algorithm
for the row-based and non-zero based SpMV schedules.
%
\autoref{fig:example-gen-code} contains code generated by our algorithm
for the row-based SpMV algorithm.

Finally, the algorithm recurses on the remainder of the
statement, and emits a distributed loop over the iteration space of the current
index variable.
%
Each point in the distributed loop is provided with all created partitions.

\begin{figure}
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gen-part-univ}
        \caption{Generated universe partition of CSR matrix for SpMV.}
        \label{fig:example-gen-parts}
    \end{subfigure}\hfill
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gen-part-coord}
        \caption{Generated non-zero partition of CSR matrix for SpMV.}
        \label{fig:example-gen-parts}
    \end{subfigure}
    \caption{Partitions of a CSR matrix created by the code generation algorithm for SpMV.}
    \label{fig:codegen-partitions}
\end{figure}

% An attempt at making a simplified version of the code generation algorithm.
% This needs another try or two.
% \begin{figure}
% \begin{lstlisting}[numbers=left]
% function codegen(IndexVar i, Statement s):
%   if i is not distributed, use TACO codegen
%   let ip be the root index variable of i
%   if i is coordinate iteration:
%     for each tensor level l accessed by ip:
%       Emit l.initUniversePartition()
%     emit loop header for i
%     for each tensor level l accessed by ip:
%       Emit l.createUniversePartitionEntry(i, {lowerBound(ip), upperBound(ip)})
%     Emit loop footer
%     for each tensor level l accessed by ip:
%       code, up, down = l.finalizeUniversePartition()
%       Emit code
%       partition coordinate tree from l using up and down
%   else: # i is position iteration
%     l = get position space tensor level
%     Emit l.initCoordinatePartition()
%     Emit loop header for i
%     Emit l.createCoordinatePartitionEntry(i, {lowerBound(ip), upperBound(ip)}
%     Emit loop footer
%     code, up, down = l.finalizeCoordinatePartition()
%     Emit code
%     partition coordinate tree from l using up and down
%     recover a universe partition from l top level partition
%     partition all other tensors using this universe partition
%   emit distributed for loop over i
%   recursively codegen(next(i), s)
% \end{lstlisting}
% \end{figure}

% An attempt at an even higher level algorithm for the codegen section.
\begin{figure}
\begin{lstlisting}[language=python]
def codegen(TINStatement s, IndexVar i):
  if not is_distributed(i):
    # Fall back to standard TACO code generation.
    taco::codegen(s, i)
  
  if coordinateValueIteration(i):
    # Create initial partitions tensors.
    createInitialUniversePartitions(i, s)
    # Derive full coordinate tree partitions.
    partitionCoordinateTrees(i, s)
  else:
    # Create initial partition of non-zero split tensor.
    createInitialNonZeroPartition(i, s)
    # Partition the full coordinate tree of the 
    # non-zero split tensor.
    partitionNonZeroCoordinateTree(i, s)
    # Using the partition of the non-zero split tensor, 
    # partition all other accessed tensors.
    partitionRemainingCoordinateTrees(i, s)
  
  # Emit a distributed for loop over the index variable and
  # pass the partitions to each iteration.
  emitDistributedForLoop(i)
  # Recursively codegen the next index variable 
  # as the loop body.
  codegen(s, next(i))
\end{lstlisting}
\end{figure}

\begin{figure}
\begin{lstlisting}[frame=single,language=Python,commentstyle=\color{gray},numbers=left, xrightmargin=0.1cm,xleftmargin=0.4cm,escapeinside={$}{$},keywords={emit, def, for, if, is, not, return, in, else}]
def partitionCoordTree(initLevel, up, down):
  for level above initLevel:
    code, up = level.partitionFromChild(up)
    emit code
  for level below initLevel:
    code, down = level.partitionFromParent(down)
    emit code
  emit `copy(down, initLevel.tensor.values)`
  return up
def codegen(IndexVar i, Statement s):
  if i is not distributed:
    taco::codegen(i, s)
    return
  # getRoot returns the root variable of i. If `j` was 
  # `divide`-ed into `jo` and `ji`, `getRoot(jo)` = `j`.
  iParent = getRoot(i)
  lo, hi = lowerBound(iParent), upperBound(iParent)
  if i is coordinate value iteration:
    partitioned = tensors in s accessed by iParent
    partitionedLevels = accessed levels of partitioned
    for level in partitionedLevels:
      emit level.initUniversePartition()
    emit `for (int i = 0; i < upperBound(i); i++) {`
    for level in partitionedLevels:
      emit level.createUniversePartitionEntry(i, {lo, hi})
    emit `}`
    for level in partitionedLevels:
      code, upPart, downPart =
         level.finalizeUniversePartition()
      emit code
      partitionCoordTree(level, upPart, downPart)
  else: # i is coordinate position iteration.
    tf = getPositionTensorLevel(s, i)
    emit tf.initCoordinatePartition()
    emit `for (int i = 0; i < upperBound(i); i++) {`
    emit tf.createCoordinatePartitionEntry(
             i, {iParentLo, iParentHi})
    emit `}`
    code, upPart, downPart = 
      tf.finalizeCoordinatePartition()
    emit code
    topPart = partitionCoordTree(tf, upPart, downPart)
    for all tensors ot != t in s:
        part = projectToUniversePart(t, topPart, ot)
        partitionCoordTree(ot, 0, None, part)
  emitDistributedForLoop(i)
  codegen(next(i), s)
\end{lstlisting}
    \caption{Code generation algorithm. Code in backticks denote  AST fragments constructed by the compiler.}
    \label{fig:codegen-alg}
\end{figure}

\begin{figure}
\begin{lstlisting}[frame=single,language=C++,commentstyle=\color{gray},numbers=left, xleftmargin=0.4cm,xrightmargin=0.1cm]
void SpMV(Tensor a, Tensor B, Tensor c, int pieces) {
  // B1.initUniversePartition()
  Coloring BColoring = {};
  for (int io = 0; io < pieces; io++) {
    int iLo = io * (B[0].dim / pieces);
    int iHi = (io + 1) * (B[0].dim / pieces);
    // B1.createUniversePartitionEntry(io, {iLo, iHi})
    BColoring[io] = {iLo, iHi - 1}; }
  // B1.finalizeUniversePartition()
  auto B1Part = partitionByBounds(B[0].dom, BColoring);
  // B2.partitionFromParent(B1Part)
  auto B2PosPart = copy(B1Part, B[1].pos);
  auto B2CrdPart = image(B2PosPart, B[1].pos);
  auto BValsPart = copy(B2CrdPart, B.vals);
  distributed for io in {0 ... pieces} {
    for (int ii = 0; ii < (B[0].dim / pieces); ii++) {
      int i = io * (B[0].dim / pieces) + ii;
        for (int jB = B[1].pos[i].lo; 
                    jB <= B[1].pos[i].hi; jB++) {
          int j = B[1].crd[jB];
          a.vals[i] += B.vals[jB] * c.vals[j];
        }}}}
\end{lstlisting}
    \caption{Generated psuedo-code for a row-based distributed SpMV operation. 
    For simplicity, partitioning of $a$ and $c$, various iteration guards 
    and bounds checks are omitted.}
    \label{fig:example-gen-code}
\end{figure}

==> old-text.tex <==


\TODO{
\section{Background}

As seen in \autoref{fig:lang-sample}, \name{} has three input sub-languages:
a \emph{computation language} that describes the desired kernel (lines \ref{fig:lang-sample:line:tensor-index-notation}),
a \emph{format language} (lines \ref{fig:lang-sample:line:dist-end}-\ref{fig:lang-sample:line:dist-end}) 
that describes how input tensors store non-zeros and are distributed onto a machine,
and a \emph{scheduling language} (lines \ref{fig:lang-sample:line:sched-begin}-\ref{fig:lang-sample:line:sched-end})
that describes how to optimize and distribute the computation.
%
In this section, we provide background on these components and detail the prior work that these abstractions draw from.

\TODO{rohany: I feel like i'm just copying the DISTAL paper right now...}

\TODO{rohany: Order the initial paragraph like the sections below.}

As discussed previously, \name{} is built on the TACO~\cite{taco} and DISTAL~\cite{TODO} compilers,
and shares their computation language called \emph{tensor index notation}.
%
Tensor index notation consists of \emph{accesses} that index tensor dimensions with lists of \emph{index variables}.
%
All statements in tensor index notation are assignments into a left-hand side access, where the right
hand side is an expression constructed from multiplication and additions between accesses.
%
As an example, third-order tensor-times-vector operation is expressed in tensor index notation
as $A(i, j) = B(i, j, k) \cdot c(k)$.
%
This notation states that each component $A(i, j)$ of the output is the result of the inner product
between the final dimension of $B$ and the vector $c$.
%
Intuitively, each distinct index variable corresponds to a nested loop, and variables contained only 
in the right-hand side of the assignment represent sum-reductions over the loop.
%
Tensor index notation allows for an arbitrary number of tensors to be present in the right-hand
side expression, and a key strength of \name{} is the ability to generate a single fused kernel
for a target tensor index notation expression.

An important component of many domain specific languages (\TODO{citations}) is
the separation of what is desired to be computed (computation language) and
how the computation should be executed.
%
This separation is canonically performed via a \emph{scheduling language},
which allow users to describe application of optimizing 
transformations while guaranteeing correctness.
%
Examples of scheduling commands defined by prior work (\TODO{citations}) include
\texttt{parallelize} (parallelize loop iterations over a hardware unit), \texttt{precompute} (hoist 
computation out of a loop), \texttt{split} (break a loop into two nested loops),
\texttt{collapse} (fuse two nested loops into a single loop), and 
\texttt{reorder} (change the ordering of loops).
%
The DISTAL~\cite{TODO} system introduced the \texttt{distribute} and
\texttt{communicate} scheduling commands to allow for scheduling tensor
computations onto distributed machines.
%
The \texttt{distribute} command indicated that iterations of the
targeted loop should execute on different nodes (or different GPUs).
%
The \texttt{communicate} command directed that the necessary subsets
of each tensor supplied to the command should be transferred between
memory spaces at the beginning of each iteration of the target loop.
%
\name{} supports all of these common scheduling directives and 
a major contribution of our work is the procedure to support DISTAL's
distributed scheduling directives for sparse tensors.

\input{distal-data-dist}

TACO and DISTAL introduced novel format languages to describe data layouts, 
with a focus on separating the computation description from the data
description, allowing users to change each independently.
%
TACO's format language allows users to control the data structure used
to compress sparse data structures by specifying a format for each dimension
in the sparse tensor.
%
This per-dimension approach allows for expression of a variety of different
common formats, as described in \TODO{Figure...}.
%
\TODO{rohany: Include fred's figures about data structure representation.}
%
For example, the common CSR matrix encoding is constructed by using a
\texttt{Dense} encoding of the first dimension and a \texttt{Compressed}
encoding of the second dimension.
%
Prior works~\cite{taco, taco_formats} detail additional format kinds and how
to represent other common sparse tensor formats using this model.
%
DISTAL's format language (called \emph{tensor distribution notation})
allowed for users to control how their tensors were
distributed onto a target abstract machine.
%
In a similar manner to TACO, tensor distribution notation allowed users to specify
how each dimension of a tensor was \emph{partitioned} onto different dimensions
of an abstract machine.
%
A tensor distribution notation statement assigned names to each dimension of a tensor
and a target machine.
%
Tensor dimensions that share a name with a machine dimension are partitioned by that
dimension of the machine.
%
A tensor distribution notation statement that maps a matrix $\mT$ onto a one-dimensional
machine $\mM$ is $\tdist{xy}{x}$.
%
This statement declares that the first dimension of $\mT$ is partitioned by the first
dimension of $\mM$, creating a row-based distribution of $\mT$.
%
We include several examples of different tensor distribution notation statements in
\autoref{fig:example-distal-data-distributions}, and point readers to the work of Yadav et al.~\cite{TODO} for 
more discussion.
%
In our work, we show how to combine these two format languages to allow for the
description of distributed sparse tensor data structures.
}

\TODO{
\section{Programming Model}

In this section, we describe \name{}'s programming model, and how it builds on the models
proposed by prior work.
%
As in DISTAL and TACO, users will describe their how their data is structured and distributed
through a format language, and will describe how their computation is distributed through
a scheduling language.

\subsection{Format Language}

\subsubsection{Sparsity Structure} \name{} adopts the per-dimension format specification of
TACO, allowing users to specialize the format of tensors to the target data and machine.
%
Logically, \name{} provides a single global view of the constructed tensor data structure,
which is partitioned to reside in the disparate memories of the target machine.
%
Concretely, consider a CSR matrix (e.g. format \texttt{Dense, Compressed}); \name{} provides
the abstraction of a single global CSR matrix data structure across all nodes.
%
Data distribution and compute operations cause different subsets of this global CSR matrix to
be materialized within and communicated between different memories.
%
\TODO{rohany: Include a figure that describes this?}

\subsubsection{Tensor Distribution Notation Extensions}

\TODO{rohany: We probably need a section (or at least a sentence or two) talking about the machine model of DISTAL.}
%
As discussed in \TODO{Section...}, tensor distribution notation allows for describing
which dimensions of a tensor $\mT$ are partitioned by dimensions of a machine $\mM$.
%
Concretely, a tensor distribution notation constructs a function that maps coordinates
of a tensor to processors in $\mM$.
%
Yadav et al. decompose this function into a pair of functions $\mP : \mT \rightarrow \textsf{color}$
and $\mF : \textsf{color} \rightarrow \mM~\textsf{set}$.
%
In this decomposition, $\mP$ is an abstract partitioning function that maps coordinates of $\mT$ into unique
colors, and $\mF$ maps these colors to processors in $\mM$.
%
For the rest of this section, we restrict our focus to the partitioning function $\mP$.

When a dimension $d$ of $\mT$ is partitioned, $\mP$ assigns a roughly equal number of coordinates
of $d$ to each distinct color.
%
When $\mT$ is a dense tensor, all coordinates of $d$ are present in $\mT$, corresponding to the
universe $\mU$, or all possible coordinate values of $d$.
%
\TODO{rohany: This previous sentence is not great$\ldots$.}
%
Thus, we denote this method of partitioning tensor coordinates as a \emph{universe partition}, as
$\mP$ can divide the total space of coordinates in $\mU$ equally.
%
When $\mT$ is sparse, the set of defined coordinates in $d$ is a subset of $\mU$, but the notion
of a universe partition still applies, as seen in \TODO{Figure...}.
%
In this partitioning, $\mU$ has been partitioning into even blocks, and the coordinates of $\mT$ that are
defined are partitioned according to the partitioning of $\mU$.
%
Universe partitions can be useful for sparse tensors (and are the default choice when using tensor distribution
notation), but can also result in imbalanced data distributions as seen in \TODO{Figure...}, as not all 
coordinates in $\mU$ may be present in $\mT$.
%
To this end, we introduce the notion of a \emph{coordinate partition}, which declares that the the partitioning
function $\mP$ should evenly partition the non-zero coordinates of a dimension $d$ instead of evenly
partitioning $\mU$.
%
A coordinate partition is invoked on a dimension name $d$ with the operator $d \downarrow \mC$ on a tensor
distribution statement.
%
For example, the tensor distribution notation statement $\tdistcoord{\mT}{x}{x \downarrow \mC}{x}$ declares
that the coordinates of a sparse vector should be distributed equally onto $\mM$.
%
\TODO{Figure ...} depicts the described coordinate partition.

For tensors with higher dimension than 1, the coordinate partition operation itself may not be enough
to achieve sufficient degrees of load balance.
%
\TODO{Figure ...} displays how the coordinate and universe partitions of a sparse matrix
can result in the same imbalanced distribution.
%
Rather than distributing the non-zero rows or non-zero columns of a matrix, it could be useful to distribute
the non-zeros of a matrix evenly instead.
%
To enable description of such data distributions, we extend tensor distribution notation with a
\emph{fusion} operator that collapses multiple dimensions into a single logical dimension, which
can then be partitioned equally.
%
The syntax $\tdistcoordfused{\mT}{xy}{xy \rightarrow f}{f \downarrow \mC}{f}$ utilizes the fusion operation
to equally distribute the non-zeros of a matrix, as seen in \TODO{Figure ...}.
%
The fusion operator introduces a new dimension name $f$, and declares that $x$ and $y$ should be collapsed to $f$.
%
Next, we declare that $f$ should be partitioned with a coordinate partition, resulting in an equal distribution
of all non-zero coordinates of the matrix.
%
\TODO{Figure ...} shows different partitioning strategies for a sparse 3-tensor using the fusion and coordinate
partition operators.

\subsection{Scheduling Language}

\name{} supports all of the distribution scheduling commands introduced by DISTAL~\cite{TODO} and
the sparse iteration space transformations in TACO~\cite{taco_scheduling}.
%
A contribution of our work is showing how these transformations can be implemented to enable
distribution of sparse tensor operations, discussed in \TODO{Section...}.
%
In this section, we highlight some important features of our scheduling system and how they
interact with distribution.

\textbf{Coordinate Tree Splitting.} Pass.

\textbf{Strip-mining Merges.} Pass.

\begin{itemize}
    \item iteration space distribution?
    \item coordinate vs pos iteration (maybe too low level)
    \item splitting the position space
    \item distributing merger loops?
\end{itemize}

\TODO{rohany: I'm not sure yet how to write this section, but I want to say that we don't
we aren't really going to change anything, but I want to highlight things like distribute
and position splits.}

\TODO{rohany: We want to also talk about the independence between how the data was distributed 
and how you can schedule the computation.}

}

